Distributed Out-of-Memory NMF on CPU/GPU Architectures

We propose an efficient distributed out-of-memory implementation of the Non-negative Matrix Factorization (NMF) algorithm for heterogeneous high-performance-computing (HPC) systems. The proposed implementation is based on prior work on NMFk, which can perform automatic model selection and extract latent variables and patterns from data. In this work, we extend NMFk by adding support for dense and sparse matrix operation on multi-node, multi-GPU systems. The resulting algorithm is optimized for out-of-memory (OOM) problems where the memory required to factorize a given matrix is greater than the available GPU memory. Memory complexity is reduced by batching/tiling strategies, and sparse and dense matrix operations are significantly accelerated with GPU cores (or tensor cores when available). Input/Output (I/O) latency associated with batch copies between host and device is hidden using CUDA streams to overlap data transfers and compute asynchronously, and latency associated with collective communications (both intra-node and inter-node) is reduced using optimized NVIDIA Collective Communication Library NCCL based communicators. Benchmark results show significant improvement, from 32X to 76x speedup, with the new implementation using GPUs over the CPU-based NMFk. Good weak scaling was demonstrated on up to 4096 multi-GPU cluster nodes with approximately 25,000 GPUs when decomposing a dense 340 Terabyte-size matrix and an 11 Exabyte-size sparse matrix of density 10e-6.

==> UserDefinedCommands.tex <==
% Place user-defined commands below.

%%%%%%%%%%%%%%%%%%%%%%%%%
%%%  DISCRETIZATION:
%%%%%%%%%%%%%%%%%%%%%%%%%
\def\dx{\triangle x}
\def\dy{\triangle y}
\def\dz{\triangle z}
\def\dt{\triangle t}
\def\dT{\triangle T}


%%%%%%%%%%%%%%%%%%%%%%%%%
%%%  OPERATORS:
%%%%%%%%%%%%%%%%%%%%%%%%%
\def\aint{\,-\hspace{-4.364mm}\int}
\def\esssup{\text{ess}\!\!\sup}
\def\Div{\operatorname{div}}
\def\lap{\triangle}
\def\trace{\operatorname{trace}}
\def\cosech{\operatorname{cosech}}
\def\cosec{\operatorname{cosec}}
\def\curl{\operatorname{curl}}
\def\Bcurl{\mathbf{curl}}


%%%%%%%%%%%%%%%%%%%%%%%%%
%%%  UNITS:
%%%%%%%%%%%%%%%%%%%%%%%%%
\def\mum{\mu\text{m}}



%%%%%%%%%%%%%%%%%%%%%%%%%
%%%  SYMBOLS:
%%%%%%%%%%%%%%%%%%%%%%%%%
\def\a{\alpha}
\def\b{\beta}
\def\d{\partial}
\def\g{\gamma}
\def\r{\rho}
\def\s{\sigma}
\def\w{\omega}
\def\l{\lambda}
\def\ve{\varepsilon}
\def\dve{\dot\varepsilon}
\def\diiv{\text{div}}

\def\G{\Gamma}
\def\D{\nabla}
\def\R{\mathbb{R}}
\def\Re{\mathcal{R}e}

\def\BSve{\boldsymbol{\varepsilon}}
\def\BSw{\boldsymbol{\omega}}
\def\BSt{\boldsymbol{\tau}}
\def\BStau{\boldsymbol{\tau}}
\def\BSa{{\boldsymbol{\alpha}}}

\def\tphi{\tilde{\phi}}


%%%%%%%%%%%%%%%%%%%%%%%%%
%%%  BOLDFACE LETTERS:
%%%%%%%%%%%%%%%%%%%%%%%%%
% SMALL
\def\Bq{\mathbf{q}}
\def\Bw{\mathbf{w}}
\def\Be{\mathbf{e}}
\def\Br{\mathbf{r}}
\def\Bt{\mathbf{t}}
\def\By{\mathbf{y}}
\def\Bu{\mathbf{u}}
\def\Bi{\mathbf{i}}
\def\Bo{\mathbf{o}}
\def\Bp{\mathbf{p}}
\def\Ba{\mathbf{a}}
\def\Bs{\mathbf{s}}
\def\Bd{\mathbf{d}}
\def\Bf{\mathbf{f}}
\def\Bg{\mathbf{g}}
\def\Bh{\mathbf{h}}
\def\Bj{\mathbf{j}}
\def\Bk{\mathbf{k}}
\def\Bl{\mathbf{l}}
\def\Bz{\mathbf{z}}
\def\Bx{\mathbf{x}}
\def\Bc{\mathbf{c}}
\def\Bv{\mathbf{v}}
\def\Bb{\mathbf{b}}
\def\Bn{\mathbf{n}}
\def\Bm{\mathbf{m}}

% CAPITAL
\def\BQ{\mathbf{Q}}
\def\BW{\mathbf{W}}
\def\BE{\mathbf{E}}
\def\BR{\mathbf{R}}
\def\BT{\mathbf{T}}
\def\BY{\mathbf{Y}}
\def\BU{\mathbf{U}}
\def\BI{\mathbf{I}}
\def\BO{\mathbf{O}}
\def\BP{\mathbf{P}}
\def\BA{\mathbf{A}}
\def\BS{\mathbf{S}}
\def\BD{\mathbf{D}}
\def\BF{\mathbf{F}}
\def\BG{\mathbf{G}}
\def\BH{\mathbf{H}}
\def\BJ{\mathbf{J}}
\def\BK{\mathbf{K}}
\def\BL{\mathbf{L}}
\def\BZ{\mathbf{Z}}
\def\BX{\mathbf{X}}
\def\BC{\mathbf{C}}
\def\BV{\mathbf{V}}
\def\BB{\mathbf{B}}
\def\BN{\mathbf{N}}
\def\BM{\mathbf{M}}

%%%%%%%%%%%%%%%%%%%%%%%%%
%%%  CAL SPACES:
%%%%%%%%%%%%%%%%%%%%%%%%%
\def\cQ{\mathcal{Q}}
\def\cW{\mathcal{W}}
\def\cE{\mathcal{E}}
\def\cR{\mathcal{R}}
\def\cT{\mathcal{T}}
\def\cY{\mathcal{Y}}
\def\cU{\mathcal{U}}
\def\cI{\mathcal{I}}
\def\cO{\mathcal{O}}
\def\cP{\mathcal{P}}
\def\cA{\mathcal{A}}
\def\cS{\mathcal{S}}
\def\cD{\mathcal{D}}
\def\cF{\mathcal{F}}
\def\cG{\mathcal{G}}
\def\cH{\mathcal{H}}
\def\cJ{\mathcal{J}}
\def\cK{\mathcal{K}}
\def\cL{\mathcal{L}}
\def\cZ{\mathcal{Z}}
\def\cX{\mathcal{X}}
\def\cC{\mathcal{C}}
\def\cV{\mathcal{V}}
\def\cB{\mathcal{B}}
\def\cN{\mathcal{N}}
\def\cM{\mathcal{M}}


%%%%%%%%%%%%%%%%%%%%%%%%%
%%%  MATRICES:
%%%%%%%%%%%%%%%%%%%%%%%%%
\def\mQ{\mathbb{Q}}
\def\mW{\mathbb{W}}
\def\mE{\mathbb{E}}
\def\mR{\mathbb{R}}
\def\mT{\mathbb{T}}
\def\mY{\mathbb{Y}}
\def\mU{\mathbb{U}}
\def\mI{\mathbb{I}}
\def\mO{\mathbb{O}}
\def\mP{\mathbb{P}}
\def\mA{\mathbb{A}}
\def\mS{\mathbb{S}}
\def\mD{\mathbb{D}}
\def\mF{\mathbb{F}}
\def\mG{\mathbb{G}}
\def\mH{\mathbb{H}}
\def\mJ{\mathbb{J}}
\def\mK{\mathbb{K}}
\def\mL{\mathbb{L}}
\def\mZ{\mathbb{Z}}
\def\mX{\mathbb{X}}
\def\mC{\mathbb{C}}
\def\mV{\mathbb{V}}
\def\mB{\mathbb{B}}
\def\mN{\mathbb{N}}
\def\mM{\mathbb{M}}



% TEXT (in formulas)
\def\CA{\mathcal{A}}
\def\TA{\text{A}}
\def\TB{\text{B}}
\def\TC{\text{C}}





==> mark.tex <==
We would like to thank the Reviewers for their valuable comments and recommendations for improving the manuscript. We carefully considered all the points raised by the Reviewers which we believe have helped identify potential sources of confusion that need clarification. In the interest of keeping our reply to 1000 words we are only dressing major concerns bellow. All minor concerns will be included  in the revised manuscript.
## Reviewer-1
##### (1)
* In algorithm 1, \(@\) and \(\epsilon\) respectively designate matrix multiplication a small floating point number(\(\sim 10^{-8}\)). A nomenclature for both \(@\) and \(\epsilon\) will be incorporated in the revised manuscript.
- We have used NCCL's version of All\_reduce(AR); the details of the implementation are in[5,6,7,8]. Regarding NCCL vs. MPI performance, the reader is referred to[7] for benchmarks and detailed comparative study.
- We agree with the Reviewer of the need for clarification for intermediate AR of sub-products. Here the compute of \(AHT_p\) involves two steps, as explained in Algorithm 3: First we compute the sub-product \(AHT_p \leftarrow A_p @ HT\) which is local to each GPU, and second the full product \(AHT_p\) is obtained by adding all the different sub-products from the different GPUs using the AR as follows \(AHT_p \leftarrow \operatorname{\text{All\_Reduce}}(AHT_p)\), which is an intermediate value for the update of \(W\).
##### (2)
* We believe the CPU implementation(pyDNMFk) is efficient because its performance was demonstrated with published bench-marking results[11,12]. Further, our GPU implementation closely follows the CPU implementation, where the major difference is the added new features for batching and communication using NCCL. Results in figures(3(a)-3(b)) were obtained without the batching feature which effectively means that very similar algorithms were run on both GPU and CPU with the difference of  NCCL handling communication in the GPU implementation and MPI in the CPU implementation.
* We agree with the reviewer of the need for clarification on the discussion of results. The results presented in figures(3(a)-3(b)) only compare the speedup gain associated with AR communication time, and does not include any compute time. Since the CPU implementation uses MPI for communication, and GPU implementation uses NCCL, we are essentially only comparing the communication time of MPI to that of NCCL. Consequently the observed \(100X\) improvement is an indication of communication speed up using NCCL compared to MPI.

## Reviewer-2
##### Weaknesses-1,2,4, and questions-1,2,3
* The use of NCCL to reduce communication cost in distributed algorithms is not novel; however, this is the first time NCCL is used in NMF implementation. 
* To the best of our knowledge, the only existing implementation that potentially has some form of multi-node multi-GPU distributed implementation of NMF, PLANC[14], but does not offer benchmark results to compare against. On the other hand, a comparison with other existing implementations would have to be in the single node configuration, which does not provide useful insights into the efficiency of our approach, as a good performance in a single node configuration does not translate into a good performance in a distributed system(where other issues such as inter-node communication are bottlenecks).
* Only PLANC[14] uses inter-node communication with MPI, and the remaining existing single node implementations of NMF are not distributed, and do not use inter-node communication.
* Compared to other CPU NMF implementations, pyDNMFk is a good choice because it is a distributed algorithm that demonstrated good scaling performance across more than 25k CPUs and large datasets. Above all, pyDNMFk-GPU inherits the capabilities for automatic model determination from pyDNMFk, which does not exist in other distributed GPU NMF implementations.
##### Weakness-3
* We use synthetic datasets because we try to show the ability of our method to find the number of latent features, and for synthetic datasets we know the ground truth. Differently, we often do not know the true number of latent features in real-world data. Therefore, we can not evaluate the performance of automatic model determination. This puts working on large scale real world data in an exploratory analysis work requiring Domain Experts which is outside the scope of our work.
*  Figures(3a,3b) compare two aspects of the algorithm. Figure(3a) shows the speedup gain on computation alone, while Figure(3b) shows speedup gain on communication alone. Figure(3a) shows the difference in hardware computation capabilities, and Figure(3b) gives insight on communication improvements achieved by the use of NCCL, as explained above.
#### Questions-4,6
 * NCCL and out-of-core are not closely related: NCCL is a communication library(similar to MPI), which we use to speed up communication. Out-of-core is an implementation design that enables us to handle big data at scales that do not fit in available memory at once.
* Out-of-core implementation comes with drawbacks due to the employed batching techniques, which breaks large communications into multiple smaller communication loads that each come with overhead cost(Section-3.2). These overheads add up when the number of batches is large, in which case using NCCL is helpful because of the reduced communication overhead costs. We also overlap communication and compute to hide some of the overhead cost(Section-3.1).
##### Question-5
In the revised manuscript we will include the following explanation: "The decrease in performance with increasing \(k\), when \(k > 32\), is explained by the compute complexity \(\mathcal{O}_c(k \times J \times I)\) of the proposed algorithm(Section-3.3). It can be seen that complexity grows with the size of \(k\) for a fixed \(I\) and \(J\)".

## Reviewer-3
##### Question-1
* We will refine this section in the final version of the paper to ensure the information regarding the complexity of the algorithms are communicated clearly. 
* The citation for pyDNMFk are[11,12]. Please be advised that[11] is for the official pyDNMFk GitHub repository: https://github.com/lanl/pyDNMFk

## Reviewer-4
##### Question-1
To the best of our understanding of the NMF algorithm, a distributed implementation without any all-reduce communication is not feasible. The best we are able to offer is an implementation that avoids all-reduce communications in only one of the two factor updates in NMF. In CNMF AR is avoided in the H-update, and similarly, AR is avoided in the W-update in RNMF. Further saving in AR is proposed in the form of choice of CNMF(when \(m>n\) or RNMF(when \(n>m\) (Section-3.1).

%Because of the shear amount of questions related to NCCL, we propose to add a subsection with the following discussion on NCCL:
%The NVIDIA Collective Communications Library(NCCL) is an open-source library providing inter-GPU communication primitives developed and maintained by NVIDIA. NCCL performs automatic hardware topology detection, which it then uses in graph search algorithms to identify communication paths that offer the highest bandwidth and lowest latencies for communication between GPUs intra- and inter-node(e.g., between GPUs that are on the same compute node, as well as between GPUs that are on separate compute nodes). NCCL is compatible with many multi-GPU parallelization models, and provides the ability to perform MPI-like collective and point-to-point operations such as allgather, reduce, broadcast, AR, send, and recv. NCCL was initially proposed to help with the need to efficiently transfer large message GPU buffers in deep learning applications. Many leading deep learning frameworks like Chainer, PyTorch, and TensorFlow have since integrated NCCL to accelerate deep learning training on multi-GPU, multi-node systems, which has motivated us to use NCCL to handle communication in our proposed NMF implementation.

